One-out-of-Many Unclonable Cryptography: Definitions, Constructions, and More

The no-cloning principle of quantum mechanics enables us to achieve amazing unclonable cryptographic primitives, which is impossible in classical cryptography. However, the security definitions for unclonable cryptography are tricky. Achieving desirable security notions for unclonability is a challenging task. In particular, there is no indistinguishable-secure unclonable encryption and quantum copy-protection for single-bit output point functions in the standard model. To tackle this problem, we introduce and study relaxed but meaningful security notions for unclonable cryptography in this work. We call the new security notion one-out-of-many unclonable security. We obtain the following results. - We show that one-time strong anti-piracy secure secret key single-decryptor encryption (SDE) implies one-out-of-many indistinguishable-secure unclonable encryption. - We construct a one-time strong anti-piracy secure secret key SDE scheme in the standard model from the LWE assumption. - We construct one-out-of-many copy-protection for single-bit output point functions from one-out-of-many indistinguishable-secure unclonable encryption and the LWE assumption. - We construct one-out-of-many unclonable predicate encryption (PE) from one-out-of-many indistinguishable-secure unclonable encryption and the LWE assumption. Thus, we obtain one-out-of-many indistinguishable-secure unclonable encryption, one-out-of-many copy-protection for single-bit output point functions, and one-out-of-many unclonable PE in the standard model from the LWE assumption. In addition, our one-time SDE scheme is the first SDE scheme that does not rely on any oracle heuristics and strong assumptions such as indistinguishability obfuscation and witness encryption.

==> OT_SDE_LWE_new.tex <==
% !TEX root = main.tex

\renewcommand{\msglen}{\ell}
\newcommand{\tlO}{\tilde{O}}
\newcommand{\CC}{\mathsf{CC}}
\newcommand{\qSDKG}{\qalgo{SDKG}}
\newcommand{\SDEnc}{\algo{SDEnc}}
\newcommand{\qSDDec}{\qalgo{SDDec}}
\newcommand{\sdct}{\mathsf{sdct}}
\newcommand{\tlE}{\tilde{E}}

\newcommand{\NQANLG}{\algo{NQANLG}}
\newcommand{\Htrans}[1]{{#1}^\dagger}


\section{One-Time Secure Single-Decryptor Encryption from LWE}\label{sec:ot_SDE_LWE}

We present one-time secure single-decryptor secret key encryption schemes in this section.

\subsection{Definitions}\label{sec:def_secret-key_SDE}

\begin{definition}[Single-Decryptor Secret Key Encryption (Syntax)]\label{def:sd_ske}
A single-decryptor secret key encryption scheme $\SDE$ is a tuple of quantum algorithms $(\qKG,\Enc,\qDec)$ with plaintext space $\Ms$.
\begin{description}
    \item[$\qKG (1^\secp) \ra (\ek,\qdk)$:] The key generation algorithm takes as input the security parameter $1^\secp$ and outputs an encryption key $\ek$ and a quantum decryption key $\qdk$.
    \item[$\Enc(\ek,m) \ra \ct$:] The encryption algorithm takes as input $\ek$ and a plaintext $m\in\Ms$ and outputs a ciphertext $\ct$.
    \item[$\qDec(\qdk,\ct) \ra m^\prime$:] The decryption algorithm takes as input $\qdk$ and $\ct$ and outputs a plaintext $m^\prime \in \Ms$ or $\bot$.

\item[Decryption correctness:] There exists a negligible function $\negl$ such that for any $m\in\Ms$, 
\begin{align}
\Pr\left[
\qDec(\dk,\ct)= m
\ \middle |
\begin{array}{ll}
(\ek,\qdk)\gets \qKG(1^\secp)\\
\ct \gets \Enc(\ek,m)
\end{array}
\right] 
=1-\negl(\secp).
\end{align}

\end{description}
\end{definition}


\begin{definition}[Encryption Key Reveal Strong Anti-Piracy Security]\label{def:ek_santi_piracy}
Let $\gamma\in[0,1]$. Let $\SDE=(\qKG,\Enc,\qDec)$ be a single-decryptor secret key encryption scheme. We consider the encryption key reveal strong anti-piracy game $\expc{\SDE,\qA}{ek}{santi}{piracy}(\secp,\gamma)$ between the challenger and an adversary $\qA=(\qA_0,\qA_1,\qA_2)$ below.
\begin{enumerate}
\item The challenger generates $(\ek,\qdk) \gets \qKG(1^\secp)$ and sends $\qdk$ to $\qA_0$.
\item $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA$ sends $(m_0,m_1)$, $\qstateq[\qreg{R}_1]$, and $\qstateq[\qreg{R}_2]$ to the challenger, $\qA_1$, and $\qA_2$, respectively.

\item The challenger sends $\ek$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $\pirateD_1=(\rho[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\rho[\qreg{R}_2],\mat{U}_2)$.

\item The challenger runs the test for a $\gamma$-good decryptor with respect to $(m_0,m_1)$ on $\pirateD_1$ and $\pirateD_2$. The challenger outputs $1$ if both tests pass and outputs $0$ otherwise.
\end{enumerate}

We say that $\SDE$ is one-time strong anti-piracy secure if for any $\gamma\in[0,1]$ and QPT adversary $\qA$, it satisfies that
\begin{align}
\advc{\SDE,\qA}{ek}{santi}{piracy}(\secp)\seteq\Pr[ \expc{\SDE,\qA}{ek}{santi}{piracy}(\secp, \gamma)=1]= \negl(\secp).
\end{align}
\end{definition}
\ryo{will explain the definitional choice.}

\subsection{Construction from LWE}\label{sec:construction_sk_SDE_from_LWE}

\begin{definition}[Canonical Representative of a Coset~\cite{C:CLLZ21}]
For a subspace $A$, we define the function $\Can{A}$ such that $\Can{A}(s)$ is the lexicographically smallest vector contained in $A+s$ (we call this the canonical representative of coset $A+s$).
\end{definition}

\begin{fact}[\cite{C:CLLZ21}]\label{fact:canonical_rep_coset}
If $\tilde{s}\in A+s$, then $\Can{A}(s)=\Can{A}(\tilde{s})$.
In addition, if we have the description of $A$, we can compute $\Can{A}$ in polynomial-time.
\end{fact}

We use the following tools:
\begin{itemize}
\item Garbling scheme $\GC=(\Garble,\Eval)$.
\item Hash encryption $\HE=(\HKG,\Hash,\HEnc,\HDec)$.
\item PKE with sub-exponentially unpredictable seeds $\PKE=(\KG,\Enc,\Dec)$.
\end{itemize}

The description of $\SDE$ is as follows. The plaintext space of $\SDE$ is $\bit^\msglen$.
In the following, the notations $\{X_{j,\alpha}\}_{j,\alpha}$ and $\{X_j\}_{j}$ are the abbreviations for $\{X_{j,\alpha}\}_{j\in [n],\alpha \in \bin}$ and $\{X_j\}_{j \in [n]}$, respectively.
\begin{description}

 \item[$\qSDKG(1^\secp)$:] $ $
 \begin{itemize}
\item Sample random $n/2$-dimensional subspace $A\subseteq \bbF_2^n$, where $n$ is a polynomial of $\secp$ specified later.
\item Generate two uniformly random vectors $s_1,s_2\la\bbF_2^n$.
%\item Genrate $\tlP_1\la\CCOEObf(1^\secp,\Can{A},\Can{A}(s_1))$ and  $\tlP_2\la\CCOEObf(1^\secp,\Can{A},\Can{A}(s_2))$.
\item Generate the coset state $\ket{A_{s_1,s_2}}$.
\item Generate $\hk\la\HKG(1^\secp,1^n)$.
\item Compute $\sk_1\la\Can{A}(s_1)$ and $\sk_2\la\Can{A^\perp}(s_2)$.
\item Compute $h_1\la \Hash(\hk,\sk_1)$ and $h_2\la\Hash(\hk,\sk_2)$.
\item Output $\ek:=(A,\hk,h_1,h_2)$ and $\dk:=\ket{A_{s_1,s_2}}$.
 \end{itemize}
 \item[$\SDEnc(\ek,m)$:] $ $
 \begin{itemize}
 \item Parse $\ek = (A,\hk,h_1,h_2)$.
 \item Generate $2$-out-of-$2$ secret shares $\share_1$ and $\share_2$ (i.e., random $\share_1,\share_2\in\bit^\msglen$ such that $\share_1\oplus \share_2=m$).
 \item Let $C[\share,R]$ be a circuit that has $\share,R$ hardwired, and on input $\sk$ compute $\pk\la\KG(\sk)$ and outputs $\ct\la\Enc(\pk,\share;R)$.
 \item Generate $(\tlC_1,\{\lbl_{1,j,\alpha}\}_{j,\alpha})\la\Garble(1^\secp,C[\share_1,R_1])$ and $(\tlC_2,\{\lbl_{2,j,\alpha}\}_{j,\alpha})\la\Garble(1^\secp,C[\share_2,R_2])$, where $R_1$ and $R_2$ are random coins.
 \item Generate $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j,\alpha})$ and $\hct_{2,j,\alpha}\la\HEnc(\hk,(h_2,j,\alpha),\lbl_{2,j,\alpha})$ for every $j\in[n]$ and $\alpha\in\bit$.
 \item Output $\sdct :=(A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
 \end{itemize}
\item[$\qSDDec(\qdk,\sdct)$:] $ $
\begin{itemize}
\item Parse $\qdk =\ket{A_{s_1,s_2}}$ and $\ct = (A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
\item Compute $\sk_1=\Can{A}(s_1)$ from $\ket{A_{s_1,s_2}}$ and $A$.\fuyuki{I think this can be done without destroying $\ket{A_{s_1,s_2}}$. This is because $\Can{A}(x)=\Can{A}(s_1)$ for any $x\in A+s_1$.}
\ryo{It follows from~\cref{fact:canonical_rep_coset}.}
\item Compute $\sk_2=\Can{A^\perp}(s_2)$ from $\ket{A_{s_1,s_2}}$ and $A$.
\item Compute $\lbl_{1,j}\la\HDec(\hk,\sk_1,\hct_{1,j,\sk_1[j]})$ and  $\lbl_{2,j}\la\HDec(\hk,\sk_2,\hct_{2,j,\sk_2[j]})$ for every $j\in[n]$.
\item Compute $\ct_1\la\Eval(\tlC,\{\lbl_{1,j}\}_j)$ and $\ct_2\la\Eval(\tlC,\{\lbl_{2,j}\}_j)$.
\item Compute $\share_1^\prime\la\Dec(\sk_1,\ct_1)$ and $\share_2^\prime\la\Dec(\sk_2,\ct_2)$.
\item Output $m:=\share_1^\prime\oplus \share_2^\prime$.
\end{itemize}
\end{description}


\begin{theorem}\label{thm:SDE_from_MOE_MICCObf}
If $\GC$, $\HE$, and $\PKE$ are secure, and the strong monogamy property holds,  $\SDE$ is a one-time strong anti-piracy secure single-decryptor SKE.
\end{theorem}
\begin{proof}
Let $\gamma\in[0,1]$ and $\qA=(\qA_0,\qA_1,\qA_2)$ be any QPT adversary. 
We consider sequence of games where the first game Game $1$ is $\expc{\SDE,\qA}{ot}{santi}{piracy}(\secp,\gamma)$.
\begin{description}
\item[$\hybi{1}$:] This is $\expc{\SDE,\qA}{ot}{santi}{piracy}(\secp,\gamma)$. The concrete description is as follows.
\begin{enumerate}
\item The challenger generates $(\ek,\qdk)$ as follows.
\begin{itemize}
\item Sample random $n/2$-dimensional subspace $A\subseteq \bbF_2^n$, where $n$ is a polynomial of $\secp$ specified later.
\item Generate two uniformly random vectors $s_1,s_2\la\bbF_2^n$.
%\item Genrate $\tlP_1\la\CCOEObf(1^\secp,\Can{A},\Can{A}(s_1))$ and  $\tlP_2\la\CCOEObf(1^\secp,\Can{A},\Can{A}(s_2))$.
\item Generate the coset state $\ket{A_{s_1,s_2}}$.
\item Generate $\hk\la\HKG(1^\secp,1^n)$.
\item Compute $\sk_1\la\Can{A}(s_1)$ and $\sk_2\la\Can{A^\perp}(s_2)$.
\item Compute $h_1\la \Hash(\hk,\sk_1)$ and $h_2\la\Hash(\hk,\sk_2)$.
\item Output $\ek:=(A,\hk,h_1,h_2)$ and $\dk:=\ket{A_{s_1,s_2}}$.
\item Set $\ek:=(A,\hk,h_1,h_2)$ and $\qdk:=\ket{A_{s_1,s_2}}$.
\end{itemize}
The challenger sends $\qdk$ to $\qA$.
\item $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA$ sends $(m_0,m_1)$, $\qreg{R}_1$, and $\qreg{R}_2$ to the challenger, $\qA_1$, and $\qA_2$, respectively.

\item The challenger sends $\ek$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $\pirateD_1=(\qreg{R}_1,\mat{U}_1)$ and $\pirateD_2=(\qreg{R}_2,\mat{U}_2)$, where $\qreg{R}_1$ and $\qreg{R}_2$ have a possibly entangled quantum state $\rho$, and $\mat{U}_i=(\mat{U}_{i,c})_c$ for $i\in\{1,2\}$.

\item For $i\in\{1,2\}$, let $\mat{P}_{i}=(\mat{P}_{i,b,c},\mat{I}-\mat{P}_{i,b,c})_{b,c}$ be a collection of binary projective measurements where
\begin{align}
\mat{P}_{i,b,c}=\mat{U}_{i,c}^\dagger\ket{b}\bra{b}\mat{U}_{i,c}.
\end{align}
We also define $D$ as the distribution that generates $b\la\bit$ and $c\la\Enc(\ek,m_b)$ and outputs $(b,c)$.
Also, for $i\in\{1,2\}$, we denote the mixture of $\mat{P}_i$ with respect to $D$ as $\mat{P}_{i,D}$.
The challenger applies $\TI_{\frac{1}{2}+\gamma}(\mat{P}_{1,D})$ and $\TI_{\frac{1}{2}+\gamma}(\mat{P}_{2,D})$ to $\qreg{R}_1$ and $\qreg{R}_2$, respectively.
The challenger outputs $1$ if both outcomes are $1$ and outputs $0$ otherwise.
\end{enumerate}
\end{description}

We let $\SUC_j$ be the event that the output of $\hybi{j}$ is $1$.



\begin{description}
\item[$\hybi{2}$:] This game is the same as $\hybi{1}$ except that the challenger applies $\ATI^{\epsilon,\delta}_{\mat{P}_{i},D,\frac{1}{2}+\gamma}$ instead of $\TI_{\frac{1}{2}+\gamma}(\mat{P}_{i,D})$ to $\qreg{R}_i$ for $i\in\{1,2\}$, and outputs $1$ if both outcomes are $1$ and outputs $0$ otherwise, where $\epsilon=\gamma/4$ and $\delta$ is a negligible function of $\secp$.
\end{description}
From \cref{lem:ATI_bipartite_app}, $\Pr[\SUC_2]\ge\Pr[\SUC_1]-2\delta$.

In the rest of the proof, we prove that $\Pr[\SUC_2]$ is negligible.
To this end, we assume that $\Pr[\SUC_2]$ is non-negligible.
We let $\sigma$ be the state after applying $\ATI^{\epsilon,\delta}_{\mat{P}_{1},D,\frac{1}{2}+\gamma}\tensor\ATI^{\epsilon,\delta}_{\mat{P}_{2},D,\frac{1}{2}+\gamma}$ to $\rho$ conditioned on both outcomes being $1$.
From \cref{lem:ATI_bipartite_app}, we have
\begin{align}
 \Tr[(\TI_{\frac{1}{2}+\frac{\gamma}{2}}(\cP_{1,D})\tensor \TI_{\frac{1}{2}+\frac{\gamma}{2}}(\cP_{2,D})) \sigma] \ge 1-4\delta.
\label{eqn:SDE_bipartite}
 \end{align}
%We show that we can extract $s_1$ from $\qreg{R}_1$ and then extract $s_2$ from $\qreg{R}_2$ if we have $\sigma$ satisfying \cref{eqn:SDE_bipartite}.
We define the following distribution $D^\prime$.
\begin{description}
\item[$D^\prime$:] It first generates $b\la\bit$. It then generates $(b,c)$, where $c$ is generated as follows.
\begin{itemize}
 \item Generate $2$-out-of-$2$ secret shares $\share_1$ and $\share_2$ (i.e., random $\share_1,\share_2\in\bit^\msglen$ such that $\share_1\oplus \share_2=m$).
 \item Generate $\ct_1\la\Enc(\pk_1,\share_1)$ and $\ct_2\la\Enc(\pk_2,\share_2)$.
 \item Generate $(\tlC_1,\{\lbl_{1,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_1)$ and $(\tlC_2,\{\lbl_{2,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_2)$.
 \item Generate $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j})$ and $\hct_{2,j,\alpha}\la\HEnc(\hk,(h_2,j,\alpha),\lbl_{2,j})$ for every $j\in[n]$ and $\alpha\in\bit$.
 \item Set $c :=(A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
\end{itemize}
\end{description}
$D$ and $D^\prime$ are computationally indistinguishable from the security of $\GC$ and $\HE$.
We prove it as \cref{lem:ind_D_Dprime} at the end of this proof.
Thus, from \cref{cor:ind_distribution_ATI}, we have
\begin{align}
 \Tr[(\TI_{\frac{1}{2}+\frac{\gamma}{4}}(\cP_{1,D^\prime})\tensor \TI_{\frac{1}{2}+\frac{\gamma}{4}}(\cP_{2,D^\prime})) \sigma] \ge 1-\negl(\secp).
\label{eqn:SDE_bipartite_dprime}
 \end{align}






\paragraph{Extraction from $\qreg{R}_1$.}
From \cref{eqn:SDE_bipartite_dprime}, we have
\begin{align}
\Tr[(\TI_{\frac{1}{2}+\frac{\gamma}{4}}(\cP_{1,D^\prime})\tensor \mat{I})\sigma]\ge 1-\negl(\secp).
\end{align}
This implies that 
\begin{align}
\Tr[(\mat{P}_{1,D^\prime}\tensor \mat{I})\sigma]\ge \frac{1}{2}+\frac{\gamma}{4}-\negl(\secp).
\label{eqn:SDE_R1_Dprime}
\end{align}

We consider the following distribution $D_1^\prime$.
\begin{description}
\item[$D_1^\prime$:] It generates $b\la\bit$. it outputs $(b,c)$, where $c$ is generated as follows.
\begin{itemize}
 \item Generate $\share_2\la\bit^\msglen$.
 \item Generate $\ct_1\la\Enc(\pk,0^\msglen)$ and $\ct_2\la\Enc(pk_2,\share_2)$.
 \item Generate $(\tlC_1,\{\lbl_{1,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_1)$ and $(\tlC_2,\{\lbl_{2,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_2)$.
 \item Generate $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j})$ and $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j})$ for every $j\in[n]$ and $\alpha\in\bit$.
 \item Set $c :=(A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
\end{itemize}
\end{description}
Then, letting $\mat{P}_{1,D_1^\prime}$ be the mixture of $\mat{P}_1$ with respect to $D_1^\prime$, it holds that
\begin{align}
\Tr[(\mat{P}_{1,D_1^\prime}\tensor \mat{I})\sigma]= \frac{1}{2}.
\label{eqn:SDE_R1_Dprimeone}
\end{align}

Consider the following distribution $\hat{D}_1$.
\begin{description}
\item[$\hat{D}_1$:]It simulates $\hybi{2}$ for $\qA$ and obtains a quantum state $\rho$ over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\ek=(A,\hk,h_1,h_2)$.
It then applies $\ATI^{\epsilon,\delta}_{\mat{P}_{1},D,\frac{1}{2}+\gamma}\tensor\ATI^{\epsilon,\delta}_{\mat{P}_{2},D,\frac{1}{2}+\gamma}$ to $\rho$, and obtains $\sigma$.
It outputs $\sk_1=\Can{A}(s_1)$ and $\qaux_1=(\ek,m_0,m_1,\sigma[\qreg{R}_1])$.
\end{description}
Under the condition that $\SUC_2$ happens in the simulated $\hybi{2}$ by $\hat{D}_1$, $(\Enc(\pk_1,\share_2\oplus m_b),\qaux_1)$ can be distinguished from $(\Enc(\pk_1,0^\msglen),\qaux_1)$ with non-negligible probability from \cref{eqn:SDE_R1_Dprime,eqn:SDE_R1_Dprimeone} and \cref{thm:ind_distribution_TI}, where $(\sk_1,\qaux_1)\la \hat{D}_1$. 
Since we now assume that $\Pr[\SUC_2]$ is non-negligible, $(\Enc(\pk_1,\share_2\oplus m_b),\qaux_1)$ can be distinguished from $(\Enc(\pk_1,0^\msglen),\qaux_1)$ with non-negligible probability.
By assuming $\PKE$ satisfies semantic security, this implies that $\hat{D}_1$ is not a sub-exponentially unpredictable distribution. From this fact, there exists an extraction process $\cM_1$ that computes $\sk_1$ from $\qaux_1$ with probability significantly greater than inverse sub-exponential, where $(\sk_1,\qaux_1)\la\hat{D}_1$.

\paragraph{Extraction from $\qreg{R}_2$.}
We first introduce the following lemma shown by \cite{C:CLLZ21}.
\begin{lemma}[\cite{C:CLLZ21}]\label{lem:good_dec}
Let $\rho$ be a bipartite state on registers $\qreg{R}_1$ and $\qreg{R}_2$. Let $\mat{U}_1$ and $\mat{U}_2$ be general quantum circuits acting respectively on $\qreg{R}_1$ and $\qreg{R}_2$. Suppose that $(\rho[\qreg{R}_1],\mat{U}_1)$ and $(\rho[\qreg{R}_2,\mat{U}_2)$ are both $\gamma$-good decryptors with respect to a distribution $D$ over pairs of (bit, ciphertext). Let $\cM$ be any POVM on $\qreg{R}_1$. Then, the post-measurement state on $\qreg{R}_2$ (together with $\mat{U}_2$) conditioned on any outcome is still a $\gamma$-good decryptor with respect to distribution $D$.
\end{lemma}

Let $\sigma^\prime$ be the state after applying $\cM_1$ to $\sigma$.
From \cref{eqn:SDE_bipartite_dprime,lem:good_dec}, we have
\begin{align}
\Tr[(\mat{I}\tensor\TI_{\frac{1}{2}+\frac{\gamma}{4}}(\cP_{2,D^\prime}))\sigma^\prime]\ge 1-\negl(\secp).
\end{align}
and thus
\begin{align}
\Tr[(\mat{I}\tensor\mat{P}_{2,D^\prime})\sigma]\ge \frac{1}{2}+\frac{\gamma}{4}-\negl(\secp).
\label{eqn:SDE_R2_Dprime}
\end{align}

We consider the following distribution $D_2^\prime$.
\begin{description}
\item[$D_2^\prime$:] It generates $b\la\bit$. it outputs $(b,c)$, where $c$ is generated as follows.
\begin{itemize}
 \item Generate $\share_1\la\bit^\msglen$.
 \item Generate $\ct_1\la\Enc(\pk_1,\share_1)$ and $\ct_2\la\Enc(\pk_2,0^\msglen)$.
 \item Generate $(\tlC_1,\{\lbl_{1,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_1)$ and $(\tlC_2,\{\lbl_{2,j}\}_{j})\la\GC.\Sim(1^\secp,\abs{\Enc},\ct_2)$.
 \item Generate $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j})$ and $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j})$ for every $j\in[n]$ and $\alpha\in\bit$.
 \item Set $c :=(A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
\end{itemize}
\end{description}
Then, letting $\mat{P}_{2,D_2^\prime}$ be the mixture of $\mat{P}_2$ with respect to $D_2^\prime$, it holds that
\begin{align}
\Tr[(\mat{I}\tensor\mat{P}_{2,D_2^\prime})\sigma]= \frac{1}{2}.
\label{eqn:SDE_R2_Dprimetwo}
\end{align}

Consider the following distribution $\hat{D}_2$ and QPT algorithm $\qB_2$.
\begin{description}
\item[$\hat{D}_2$:]It simulates $\hybi{2}$ for $\qA$ and obtains a quantum state $\rho$ over registers $\qreg{R}_1$ and $\qreg{R}_2$, and $\ek=(A,\hk,h_1,h_2)$.
It then applies $\ATI^{\epsilon,\delta}_{\mat{P}_{1},D,\frac{1}{2}+\gamma}\tensor\ATI^{\epsilon,\delta}_{\mat{P}_{2},D,\frac{1}{2}+\gamma}$ to $\rho$, and obtains $\sigma$.
It also applies $\cM_1$ to $\qaux_1=(\ek,m_0,m_1,\sigma[\qreg{R}_1])$, and obtains $\sigma^\prime$.
It outputs $\sk_2=\Can{A^\perp}(s_2)$ and $\qaux_2=(\ek,m_0,m_1,\sigma^\prime[\qreg{R}_2])$.
\end{description}
Under the condition that $\SUC_2$ happens in the simulated $\hybi{2}$ by $\hat{D}_2$, $(\Enc(\pk_2,\share_1\oplus m_b),\qaux_2)$ can be distinguished from $(\Enc(\pk_2,0^\msglen),\qaux_2)$ with non-negligible probability from \cref{eqn:SDE_R2_Dprime,eqn:SDE_R2_Dprimetwo} and \cref{thm:ind_distribution_TI}, where $(\sk_2,\qaux_2)\la \hat{D}_2$. 
Since we now assume that $\Pr[\SUC_2]$ is non-negligible, $(\Enc(\pk_2,\share_1\oplus m_b),\qaux_2)$ can be distinguished from $(\Enc(\pk_2,0^\msglen),\qaux_2)$ with non-negligible probability.
By assuming $\PKE$ satisfies semantic security, this implies that $\hat{D}_2$ is not a sub-exponentially unpredictable distribution. From this fact, there exists an extraction process $\cM_2$ that computes $\sk_2$ from $\qaux_2$ with probability significantly greater than inverse sub-exponential, where $(\sk_2,\qaux_2)\la\hat{D}_2$.









\paragraph{Attacking monogamy of entanglement property.}
Consider the following experiment.
\begin{description}
\item[$\mathsf{Ext}$:]It simulates $\hybi{2}$ for $\qA$ and obtains quantum state $\rho$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. It applies $(\ATI^{\epsilon,\delta}_{\mat{P}_{1},D,\frac{1}{2}+\gamma}\tensor\ATI^{\epsilon,\delta}_{\mat{P}_{2},D,\frac{1}{2}+\gamma})$ to $\rho$. Then, it applies $\cM_i$ to $\qaux_i=(\ek, m_0,m_1,\qreg{R}_i)$, and obtains outcome $s_i^\prime$ for each $i\in\{1,2\}$, where $\ek=(A,\hk,h_1,h_2)$. It outputs $(s_1^\prime,s_2^\prime)$.
\end{description}
From the above discussions, under the assumption that $\Pr[\SUC_3]$ is non-negligible, $s_1^\prime\in A+ s_1$ and $s_2^\prime\in A+s_2$ holds for $(s_1^\prime,s_2^\prime)$ output by $\Ext$ with probability significantly greater than inverse sub-exponential.
Note that operations to $\qreg{R}_1$ and operations to $\qreg{R}_2$ commute.
Thus, this probability does not change if we change the order of operations to $\qreg{R}_1$ and $\qreg{R}_2$ as long as $\cM_1$ is applied after $\ATI^{\epsilon,\delta}_{\mat{P}_{1},D,\frac{1}{2}+\gamma}$ and $\cM_2$ is applied after $\ATI^{\epsilon,\delta}_{\mat{P}_{2},D,\frac{1}{2}+\gamma}$.


We construct the following adversary $\qB=(\qB_0,\qB_1,\qB_2)$ attacking the extended monogamy of entanglement game using $\qA$ and $\gamma$.

\begin{enumerate}
\item $\qB_0$ generates $\hk\la\HKG(1^\secp)$ and sends a function $\Leak_1(A,s_1)=\Hash(\hk,\Can{A}(s_1))$ and $\Leak_2(A,s_2)=\Hash(\hk,\Can{A^\perp}(s_2))$ to the challenger.
\item $\qB_0$ is given $\ket{A_{s_1,s_2}}$, $\Leak(A,s_1)=h_1$, and $\Leak(A,s_2)=h_2$.
\item By setting $\qdk:=\ket{A_{s_1,s_2}}$, $\qB_0$ simulates $\hybi{2}$ for $\qA_0$ and obtains $(m_0,m_1)$ and a quantum state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. Then, $\qB_0$ sends $(\gamma,\hk,h_1,h_2,m_0,m_1,\qreg{R}_1)$ to $\qB_1$ and $(\gamma,\hk,h_1,h_2,m_0,m_1,\qreg{R}_2)$ to $\qB_2$.
\item The description of $A$ is then sent to both $\qB_1$ and $\qB_2$. $\qB_1$ and $\qB_2$ behave as follows.
\begin{itemize}
\item $\qB_i$ first sets $\ek=(A,\hk,h_1,h_2)$.
Then, $\qB_i$ applies $\ATI^{\epsilon,\delta}_{\mat{P}_{i},D,\frac{1}{2}+\gamma}$ to $\qreg{R}_i$. This is possible by using $\ek$. If the outcome is $0$, $\qB_i$ outputs $\bot$. Otherwise, $\qB_i$ applies $\cM_i$ to $\qaux_i=(\ek, m_0,m_1,\qreg{R}_i)$ and outputs the outcome $s_i^\prime$.
\end{itemize}
\end{enumerate}

Wee see that the distribution of $(s_1^\prime,s_2^\prime)$ output by $\qB$ is exactly the same as that of $\Ext$. This means that $\qB$ breaks the extended monogamy of entanglement property with probability significantly greater than inverse sub-exponential, which is a contradiction.
 Thus, we can conclude that  $\Pr[\SUC_2]=\negl(\secp)$.




\begin{lemma}\label{lem:ind_D_Dprime}
$D$ and $D^\prime$ are computationally indistinguishable.
\end{lemma}

\begin{proof}
We consider the following intermediate distribution $H$ between $D$ and $D^\prime$.
\begin{description}
\item[$H$:] It first generates $b\la\bit$. It then generates $(b,c)$, where $c$ is generated as follows.
\begin{itemize}
 \item Generate $2$-out-of-$2$ secret shares $\share_1$ and $\share_2$ (i.e., random $\share_1,\share_2\in\bit^\msglen$ such that $\share_1\oplus \share_2=m$).
 \item Generate $(\tlC_1,\{\lbl_{1,j,\alpha}\}_{j,\alpha})\la\Garble(1^\secp,C[\share_1,R_1])$ and $(\tlC_2,\{\lbl_{2,j,\alpha}\}_{j,\alpha})\la\Garble(1^\secp,C[\share_2,R_2])$, where $R_1$ and $R_2$ are random coins.
 \item Generate $\hct_{1,j,\alpha}\la\HEnc(\hk,(h_1,j,\alpha),\lbl_{1,j,\sk_1[j]})$ and $\hct_{2,j,\alpha}\la\HEnc(\hk,(h_2,j,\alpha),\lbl_{2,j,\sk_2[j]})$ for every $j\in[n]$ and $\alpha\in\bit$.
 \item Set $c :=(A,\tlC_1,\{\hct_{1,j,\alpha}\}_{j,\alpha},\tlC_2,\{\hct_{2,j,\alpha}\}_{j,\alpha})$.
\end{itemize}
\end{description}
The difference between $D$ and $H$ is that $\hct_{1,j,1-\sk_1[j]}$ (resp. $\hct_{2,j,1-\sk_2[j]}$) is generated as $\HEnc(\hk,(h_1,j,1-\sk_1[j]),\lbl_{1,j,1-\sk_1[j]})$ (resp. $\HEnc(\hk,(h_2,j,1-\sk_2[j]),\lbl_{2,j,\sk_2[j]})$) in $D$ but it is generated as $\HEnc(\hk,(h_1,j,1-\sk_1[j]),\lbl_{1,j,\sk_1[j]})$ (resp. $\HEnc(\hk,(h_2,j,1-\sk_2[j]),\lbl_{2,j,\sk_2[j]})$) in $H$.
This change is justified by the security of $\HE$.
Thus, $D$ and $H$ are computationally indistinguishable.

We show that $H$ and $D^\prime$ are computationally indistinguishable from the security of $\GC$.
We have $C[\share_1,R_1](\sk_1)=\Enc(\pk_1,\share_1;R_1)$ and $C[\share_2,R_2](\sk_2)=\Enc(\pk_2,\share_2;R_2)$.
Also, in $H$, $\{\lbl_{1,j,1-\sk_1[j]}\}_j$ and $\{\lbl_{2,j,1-\sk_2[j]}\}_j$ are not used to generate an output ciphertext $c$.
Thus, by using the security of $\GC$, we can switch $(\tlC, \{\lbl_{1,j,\sk_1[j]}\}_j)$ (resp. $(\tlC, \{\lbl_{1,j,\sk_1[j]}\}_j)$) into $(\tlC_1,\{\lbl_{1,j}\}_j)\la\GC.\Sim(1^\secp,\abs{C},\Enc(\pk_1,\share_1;R_1))$ (resp.  $(\tlC_2,\{\lbl_{2,j}\}_j)\la\GC.\Sim(1^\secp,\abs{C},\Enc(\pk_2,\share_2;R_2))$).
This means $H$ and $D^\prime$ are computationally indistinguishable from the security of $\GC$.
\end{proof}

This completes the proof of~\cref{thm:SDE_from_MOE_MICCObf}.
\end{proof}

\subsection{Same-Ciphertext Anti-Piracy}\label{sec:ek_reveal_anti-piracy_same_ct}
We consider two variants of security notions for single-decryptor SKE in this section.

\begin{definition}[Encryption Key Reveal Anti-Piracy Security]\label{def:ek_anti_piracy}
Let $\SDE=(\qKG,\Enc,\qDec)$ be a single-decryptor secret key encryption scheme. We consider the one-time anti-piracy game $\expc{\SDE,\qA}{ot}{anti}{piracy}(\secp)$ between the challenger and an adversary $\qA$ below.
\begin{enumerate}
\item The challenger generates $(\ek,\qdk) \gets \qKG(1^\secp)$ and sends $\qdk$ to $\qA$.
\item $\qA$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA$ sends $(m_0,m_1)$, $\qstateq[\qreg{R}_1]$, and $\qstateq[\qreg{R}_2]$ to the challenger, $\qA_1$, and $\qA_2$, respectively.

\item The challenger chooses $\coin_i$, generates $\ct_i \gets \Enc(\ek,m_{\coin_i})$, and sends $\ek$ and $\ct_i$ to $\qA_i$ for $i\in \setbk{1,2}$.
$\qA_1$ and $\qA_2$ respectively output $\coin_1^\prime$ and $\coin_2^\prime$.
If $\coin_i^\prime = \coin_i$ for $i\in \setbk{1,2}$, the challenger outputs $1$, otherwise outputs $0$.
\end{enumerate}

We say that $\SDE$ is one-time anti-piracy secure if for any QPT adversary $\qA$, it satisfies that
\begin{align}
\advc{\SDE,\qA}{ek}{anti}{piracy}(\secp)\seteq \Pr[ \expc{\SDE,\qA}{ek}{anti}{piracy}(\secp)=1] \le \frac{1}{2} + \gamma(\secp)+ \negl(\secp).
\end{align}
\end{definition}


\begin{definition}[Encryption Key Reveal Same-Ciphertext Anti-Piracy with the Same Ciphertext Security]\label{def:ek_reveal_anti_piracy_same_ct}
Let $\SDE=(\qKG,\Enc,\qDec)$ be a single-decryptor secret key encryption scheme. We consider the encryption key reveal same-ciphertext anti-piracy game $\expd{\SDE,\qA}{ek}{anti}{piracy}{sameCT}(\secp)$ between the challenger and an adversary $\qA$ below.
\begin{enumerate}
\item The challenger generates $(\ek,\qdk) \gets \qKG(1^\secp)$ and sends $\qdk$ to $\qA$.
\item $\qA$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA$ sends $(m_0,m_1)$, $\qstateq[\qreg{R}_1]$, and $\qstateq[\qreg{R}_2]$ to the challenger, $\qA_1$, and $\qA_2$, respectively.

\item The challenger chooses $\coin \chosen \zo{}$, generates $\ct \gets \Enc(\ek,m_{\coin})$, and sends $\ek$ and $\ct$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $\coin_1^\prime$ and $\coin_2^\prime$.
If $\coin_i^\prime = \coin$ for $i\in \setbk{1,2}$, the challenger outputs $1$, otherwise outputs $0$.
\end{enumerate}

We say that $\SDE$ is encryption key reveal same-ciphertext anti-piracy secure if for any QPT adversary $\qA$, it satisfies that
\begin{align}
\advd{\SDE,\qA}{ek}{anti}{piracy}{sameCT}(\secp)\seteq \Pr[ \expd{\SDE,\qA}{ek}{anti}{piracy}{sameCT}(\secp)=1]\le \frac{1}{2}+ \gamma(\secp)+ \negl(\secp).
\end{align}
\end{definition}
The difference from~\cref{def:ek_anti_piracy} is that $\qA_1$ and $\qA_2$ receive the same $\ct \gets \Enc(\ek,m_\coin)$.
This style comes from the definition by Georgiou and Zhandry~\cite[Definition 1]{EPRINT:GeoZha20}.

We prove that the strong anti-piracy in~\cref{def:ek_santi_piracy} implies the same-ciphertext anti-piracy in~\cref{def:ek_reveal_anti_piracy_same_ct}.
We have two steps. First, we prove that the strong anti-piracy in~\cref{def:ek_santi_piracy} implies the anti-piracy in~\cref{def:ek_anti_piracy}. Second, we prove the anti-piracy in~\cref{def:ek_anti_piracy} implies the same-ciphertext anti-piracy in~\cref{def:ek_reveal_anti_piracy_same_ct}.


\paragraph{Strong anti-piracy implies anti-piracy.}
\begin{theorem}\label{thm:strong_implies_CPAstyle}
If a single-decryptor SKE scheme $\SDE$ is encryption key reveal strong anti-piracy secure, it is also encryption key reveal anti-piracy secure.
\end{theorem}
The proof of~\cref{thm:strong_implies_CPAstyle} is almost the same as the proof for single-decryptor PKE by Coladangelo et al.~\cite{C:CLLZ21}.
\ryo{Maybe we should move this to appendix since the proof is the same.}
\begin{proof}
The strong anti-piracy game is as follows.
\begin{enumerate}
\item The challenger generates $(\ek,\qdk) \gets \qKG(1^\secp)$ and sends $\qdk$ to $\qA$.
\item $\qA$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA$ sends $(m_0,m_1)$, $\qstateq[\qreg{R}_1]$, and $\qstateq[\qreg{R}_2]$ to the challenger, $\qA_1$, and $\qA_2$, respectively.

\item The challenger sends $\ek$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $\pirateD_1=(\rho[\qreg{R}_1],\mat{U}_1)$ and $\pirateD_2=(\rho[\qreg{R}_2],\mat{U}_2)$.

\item The challenger runs the test for a $\gamma$-good decryptor with respect to $(m_0,m_1)$ on $\pirateD_1$ and $\pirateD_2$. The challenger outputs $1$ if both tests pass and outputs $0$ otherwise.
\end{enumerate}
The definition of $\gamma$-good decryptor (\cref{def:test_quantum_decryptor}) and threshold implementation (\cref{def:threshold_implementation}) say the following: We can obtain $(p_1,1-p_1)$ and $(p_2, 1-p_2)$ for $\pirateD_1$ and $\pirateD_2$, respectively, by applying the projective measurement described in~\cref{def:projective_implementation}. Here $p_i$ is the decryption success probability of $\pirateD_i$. Note that we can execute the test if $\ek$ is given. Assuming $\SDE$ is encryption key reveal strong anti-piracy secure, it must hold that either $p_1 \le 1/2 + \gamma$ or $p_2 \le 1/2 +\gamma$.

The anti-piracy game is as follows.
\begin{enumerate}
\item The game is the same as above except the following test phase.
\item The challenger chooses $\coin \chosen \zo{}$, generates $\ct \gets \Enc(\ek,m_{\coin})$, and sends $\ek$ and $\ct$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $\coin_1^\prime$ and $\coin_2^\prime$.
If $\coin_i^\prime = \coin$ for $i\in \setbk{1,2}$, the challenger outputs $1$, otherwise outputs $0$.
\end{enumerate}
We can implement the test above in the anti-piracy game by using the projective measurement described in~\cref{def:projective_implementation} as follows.
The challenger applies the projective measurement and obtains $(p_1,1-p_1)$ and $(p_2, 1-p_2)$ for $\pirateD_1$ and $\pirateD_2$, respectively.
Let $S_{\pirateD_i}$ be a probability distribution that takes value $1$ with probability $p_i$ and $0$ with probability $1-p_i$ for $i \in \setbk{1,2}$.
Note that we can execute this test if $\ek$ is given.
The challenger samples $b_i \sample S_{\pirateD_i}$ for $i\in\setbk{1,2}$ and outputs $1$ if and only if $b_1=b_2=1$.
We can bound the advantage $\advc{\SDE,\qA}{ek}{anti}{piracy}(\secp)$ as follows. Let $\mathsf{Bad}$ be the event where $(p_1\ge 1/2 +\gamma) \land (p_2 \ge 1/2 + \gamma)$.
\begin{align}
\advc{\SDE,\qA}{ek}{anti}{piracy}(\secp)  = &\Pr[b_1=b_2=1\land \mathsf{Bad} ]+ \Pr[b_1=b_2=1\land \neg \mathsf{Bad}] \\
= & \Pr[b_1=b_2=1 \mid \mathsf{Bad} ] \Pr[\mathsf{Bad}] + \Pr[b_1=b_2=1 \mid \neg\mathsf{Bad}] \Pr[\neg\mathsf{Bad}]\\
\le & 1\cdot \Pr[\mathsf{Bad}] + (1/2 + \gamma) \cdot 1
\end{align}
We assume $\SDE$ encryption key reveal strong anti-piracy secure, so $\Pr[\mathsf{Bad}]$ is negligible.
Thus, $\advc{\SDE,\qA}{ek}{anti}{piracy}(\secp)$ is bounded by $1/2 + \gamma + \negl$. This completes the proof.
\end{proof}





==> implication_def.tex <==
% !TEX root = main.tex


\section{Implication to Existing Definitions}\label{sec:implication_def}

In this section, we show that our new security definitions for copy-protection imply several existing security notions.



\subsection{Implication to Distributional indistinguishability}
We first show that our simulation-based copy-protection security notions imply distributional indistinguishability, which is the security notion of compute-and-compare obfuscation.

\begin{theorem}\label{thm:cp_to_ccobf}
Let $\CP=(\qCopyProtect,\qEval)$ and $\qSim$ be a copy-protection scheme for compute-and-compare circuits and its simulator that satisfy simulation-based copy-protection security in \cref{def:sim_cp_protection} with respect to a distribution $\{D_\param\}_\param$.
Then, $\CP$ satisfies distributional indistinguishability, that is,
$$(\qCopyProtect(1^\secp,P,\lock,\msg),\qaux)\cind(\qSim(1^\secp,P.\pp,\abs{\msg}),\qaux)$$
for any $\msg$ and $\param$, where $(P,\lock,\qaux)\la D_\param$.
\end{theorem}
\begin{proof}
Suppose there exists $\qB$ who can distinguish $(\qCopyProtect(1^\secp,P,\lock,\msg),\qaux)$ from $(\qSim(1^\secp,P.\pp,\abs{\msg}),\qaux)$ with probability $\frac{1}{2}+p$ for some $\msg$, $\param$, and inverse polynomial $p$, where $(P,\lock,\qaux)\la D_\param$.
Consider the following adversary $\qA=(\qA_0,\qA_1,\qA_2)$ for the simulation-based copy-protection security of $\CP$.
On input $\rho$ and $\qaux$, $\qA_0$ gives them to $\qB$ and obtains $\qB$'s guess $\coin^\prime$, and sends it to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ just output $\coin^\prime$.
We have $\advb{\CP,\qSim,\qA}{cp}{sim}(\secp)=\frac{1}{2}+p$, which contradicts to the simulation-based copy-protection security of $\CP$.
\end{proof}

\begin{theorem}\label{thm:omcp_to_ccobf}
Let $\CP=(\qCopyProtect,\qEval,\qSim)$ and $\qSim$ be a copy-protection scheme for compute-and-compare circuits and its simulator that satisfy one-out-of-many simulation-based copy-protection security in \cref{def:om_sim_cp_protection} with respect to a distribution $\{D_\param\}_\param$.
Then, $\CP$ satisfies distributional indistinguishability, that is,
$$(\qCopyProtect(1^\secp,P,\lock,\msg),\qaux)\cind(\qSim(1^\secp,P.\pp,\abs{\msg}),\qaux)$$
for any $\msg$ and $\param$, where $(P,\lock,\qaux)\la D_\param$.
\end{theorem}
\begin{proof}
Suppose there exists $\qB$ who can distinguish $(\qCopyProtect(1^\secp,P,\lock,\msg),\qaux)$ from $(\qSim(1^\secp,P.\pp,\abs{\msg}),\qaux)$ with probability $\frac{1}{2}+p$ for some $\msg$, $\param$, and inverse polynomial $p$, where $(P,\lock,\qaux)\la D_\param$.
Consider the following $\numa=\frac{1}{p}$ tuple of adversaries $\qA=(\qA_0,\qA_1,\cdots,\qA_\numa)$ for the one-out-of-many simulation-based copy-protection security.
On input $\rho$ and $\qaux$, $\qA_0$ gives them to $\qB$ and obtains $\qB$'s guess $\coin^\prime$, and sends it to $\qA_i$ for every $i\in[\numa]$.
$\qA_i$ just outputs $\coin^\prime$ if $\alpha=i$ is chosen by the challenger.
We have $\advc{\CP,\qSim,\qA}{om}{cp}{sim}(\secp,\numa)=\frac{1}{2}+p$, which contradicts to the one-out-of-many simulation-based copy-protection security since $p>\frac{1}{2\numa}=\frac{p}{2}$.
\end{proof}

\subsection{Implications to Existing Copy-Protection Security}
We show that our simulation-based copy-protection security in \cref{def:sim_cp_protection} implies the existing copy-protection security notion first introduced by \cite{ARXIV:ColMajPor20} and have been used by many previous works~\cite{TCC:BJLPS21,TCC:AnaKal21,C:AKLLZ22}.
We focus on proving the implication for copy-protection for point functions since under the definition by \cite{ARXIV:ColMajPor20}, a copy-protection scheme for point functions can be easily transformed into one for all compute-and-compare functions.
A point functions can be described as a compute-and-compare function $\cnc{\ID}{\lock,\msg}$, where $\ID$ is the identity function.
In this section, similarly to \cite{ARXIV:ColMajPor20}, we consider a family of unpredictable distribution $D=\{D_\param\}_\param$ where each $D_\param$ outputs just $\lock$, as a family of distributions from which point functions are sampled.

In the copy-protection security by \cite{ARXIV:ColMajPor20}, we consider a security game played by a tuple of adversaries $\qA=(\qA_0,\qA_1,\qA_2)$ where given a copy protected program the task of $\qA_0$ is to generate two copies of the program for $\qA_1$ and $\qA_2$, similarly to our simulation-based copy-protection security.
$\qA_1$ and $\qA_2$ are given challenge inputs sampled from some input distribution together with copies of the program generated by $\qA_0$.
We say that $\qA$ wins if $\qA_1$ and $\qA_2$ can correctly compute the output of the program on the given challenge inputs.
The security notion requires that any $\qA$ cannot win the game with probability greater than some threshold, which is ideally set as trivial winning probability with respect to the distributions on programs and challenge inputs.
Concretely, the definition for point functions is as follows.
\begin{definition}[Copy-Protection Security for Point Functions by \cite{ARXIV:ColMajPor20}]\label{def:cp_protection_point_function_cmp}
Let $D=\{D_\param\}$, $\Dmsg=\{\Dmsg_\param\}$, and $\Dchall=\{\Dchall_{\param,\lock}\}_{\param,\lock}$ be families of distributions.
We consider the following security experiment $\expc{\CP,\qA}{cp}{pf}{cmp}(\secp)$ for $\qA=(\qA_0,\qA_1,\qA_2)$.

\begin{enumerate}
\item $\qA_0$ sends $\param$ to the challenger.
    \item The challenger generates $\lock\la D_\param$ and $\msg\la\Dmsg_\param$, generates $\rho\la\qCopyProtect(1^\secp,\ID,\lock,\msg)$, and sends $\rho$ to $\qA_0$.
    \item $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA_0$ sends $\qstateq[\qreg{R}_1]$ and $\qstateq[\qreg{R}_2]$ to $\qA_1$ and $\qA_2$, respectively.
\item The challenger generates $(x^*_1,x^*_2)\la\Dchall_{\param,\lock}$, and sends $x^*_1$ and $x^*_2$ to $\qA_1$ and $\qA_2$, respectively.

\item $\qA_1$ and $\qA_2$ respectively output $y_1$ and $y_2$.
If $y_i = \cnc{\ID}{\lock,\msg}(x_i^\ast)$ for $i\in \setbk{1,2}$, the challenger outputs $1$, otherwise outputs $0$.

\end{enumerate}
We say that $\CP$ satisfies copy-protection security for point functions with respect to $(\delta,D,\Dmsg,\Dchall)$ if for any QPT $\qA$, it holds that
\begin{align}
\advc{\CP,\qA}{cp}{pf}{cmp}(\secp)\seteq \Pr[ \expc{\CP,\qA}{cp}{pf}{cmp}(\secp)=1] \le \delta + \negl(\secp),
\end{align}
\end{definition}






Below, we consider two types of point functions separately, that is, single-bit output point functions where $\msg$ is fixed to $1$ and multi-bit output point functions where $\msg$ is a multi-bit string sampled from an unpredictable distribution.


\paragraph{Implication for single-bit output point functions.}
As the implication for the case of single-bit output point functions, we prove that simulation-based copy-protection security implies the following copy-protection security with maximally correlated challenge where $\qA_1$ and $\qA_2$ are always given the same challenge input.
\begin{definition}[Copy-Protection Security for Point Functions with Maximally Correlated Challenge]\label{def:cp_protection_point_function_mcc}
Let $D=\{D_\param\}$ be a family of distributions.
We say that a copy-protection scheme satisfies maximally correlated challenge security with respect to $D=\{D_\param\}_\param$ if it satisfies copy-protection security by \cite{ARXIV:ColMajPor20} with respect to $(\delta_w,D,\Dmsg,\Dchall_w)$ for any constant $0\le w\le 1$, where $\delta_w$, $\Dmsg$, and $\Dchall_w$ are defined as follows.
\begin{itemize}
\item $\delta=\max\{w,1-w\}$.
\item $\Dmsg$ outputs the fixed single-bit $1$.
\item $\Dchall_w=\{\Dchall_{\param,\lock}\}_{\param,\lock}$ is a family of distributions, where each $\Dchall_{\param,\lock}$ outputs $x_1^*=x_2^*=\lock$ with probability $w$ and outputs $x_1^*=x_2^*=x$ where $x$ is re-sampled from $D_\param$ with probability $1-w$.
\end{itemize}
\end{definition}
Maximally correlated challenge setting was studied by \cite{TCC:AnaKal21,C:AKLLZ22}, but \cite{C:AKLLZ22} considered a slightly different setting where $\qA_1$ and $\qA_2$ are given different re-sampled values $x_1^*\la D_\param$ and $x_2^*\la D_\param$, respectively.

\begin{theorem}
Let $D=\{D_\param\}_\param$ be a family of unpredictable distributions.
Assume $\CP$ satisfies simulation-based copy-protection security with respect to $D$.
Then, $\CP$ also satisfies copy-protection security for point functions with maximally correlated challenge with respect to $D$.
\end{theorem}

\begin{proof}
Let $\qA=(\qA_0,\qA_1,\qA_2)$ be any QPT adversary.
Also, let $0 \le w \le 1$ be a constant.
We consider the case where $1-w\le w$.
The proof when $w\le 1-w$ is similar.
We consider the following sequence of experiments.

\begin{description}
\item[$\hybi{1}$:] This is $\expc{\CP,\qA}{cp}{pf}{cmp}(\secp)$ where $\Dchall_{\param,\lock}$ outputs $x^*=\lock$ without doing re-sampling.
\begin{enumerate}
\item $\qA_0$ sends $\param$ to the challenger.
    \item The challenger generates $\lock\la D_\param$ and $\rho\la\qCopyProtect(1^\secp,\ID,\lock,\msg=1)$, and sends $\rho$ to $\qA_0$.
    \item $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$. $\qA_0$ sends $\qstateq[\qreg{R}_1]$ and $\qstateq[\qreg{R}_2]$ to $\qA_1$ and $\qA_2$, respectively.
\item The challenger sends $x^*:=\lock$ to $\qA_1$ and $\qA_2$.
$\qA_1$ and $\qA_2$ respectively output $y_1$ and $y_2$.
\end{enumerate}
\end{description}

We define the following two events.
\begin{description}
\item[$\ttAND_i$:]$y_1=1$ and $y_2=1$ in $\hybi{i}$.
\item[$\ttOR_i$:]$y_1=1$ or $y_2=1$ in $\hybi{i}$.
\end{description}

\begin{description}
\item[$\hybi{2}$:] This is the same as $\hybi{1}$ except that $\rho$ is generated as $\qSim(1^\secp, P.\pp,\abs{\msg})$, where $\qSim$ is the simulator that is guaranteed to exist by the simulation-based security of $\CP$.
\end{description}

We consider the following adversary $\qB=(\qB_0,\qB_1,\qB_2)$ that attacks $\CP$. $\qB_0$ behaves as follows.
\begin{enumerate}
\item $\qB_0$ obtains $\param$ and $\msg$ from $\qA_0$, and sends them to the challenger.
$\qB_0$ obtains $\rho$ from the challenger and sends it to $\qA_0$.
\item When $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$, $\qB_0$ sends $\qstateq[\qreg{R}_1]$ and $\qstateq[\qreg{R}_2]$ to $\qB_1$ and $\qB_2$, respectively.
\end{enumerate}
$\qB_\alpha$ for $\alpha\in\{1,2\}$ behaves as follows.
\begin{enumerate}
\item $\qB_\alpha$ send $\qstateq[\qreg{R}_\alpha]$ to $\qA_\alpha$.
\item When $\qB_\alpha$ obtains $\lock$ from the challenger, $\qB_\alpha$ sends it to $\qA_\alpha$.
\item When $\qA_\alpha$ output $y_\alpha$, it outputs $b_\alpha^\prime=0$ if $y_\alpha=1$ and $b_\alpha^\prime=1$ otherwise.
\end{enumerate}

Let the challenge bit in the security game played by $\qB$ be $b$.
If $b=0$, $\qB$ perfectly simulates $\hybi{1}$ to $\qA$.
If $b=1$, $\qB$ perfectly simulates $\hybi{2}$ to $\qA$.
Also, $\qB_1$ and $\qB_2$ output $0$ if and only if $\qA_1$ and $\qA_2$ outputs $1$, respectively.
Then, we have 
\begin{align}
\Pr[b_1^\prime=b_2^\prime=b]-\frac{1}{2}
&=\Pr[b_1^\prime= b_2^\prime=b=0]+\Pr[b_1^\prime= b_2^\prime=b=1]-\frac{1}{2}\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]+\Pr[b_1^\prime=1\land b_2^\prime=1\mid b=1])-\frac{1}{2}\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]-(1-\Pr[b_1^\prime=1\land b_2^\prime=1\mid b=1]))\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]-\Pr[b_1^\prime=0\lor b_2^\prime=0\mid b=1])\\
&=\frac{1}{2}(\Pr[\ttAND_1]-\Pr[\ttOR_2]).
\end{align}
Thus, from the simulation-based copy-protection security of $\CP$, we have $\Pr[\ttAND_1]-\Pr[\ttOR_2]\le\negl(\secp)$.


\begin{description}
\item[$\hybi{3}$:] This is the same as $\hybi{2}$ except that a re-sampled value $x^*\la D_\param$ is given to $\qA_1$ and $\qA_2$ instead of $\lock$.
\end{description}

In $\hybi{2}$, $\qA_0$ is given $\rho\la\qSim(1^\secp,\abs{\ID},\abs{\msg})$, and thus $\rho$ does not have any information of $\lock$.
Thus, we have $\Pr[\ttOR_2]=\Pr[\ttOR_3]$.

\begin{description}
\item[$\hybi{4}$:] This is the same as $\hybi{3}$ except that $\rho$ is generated as $\rho\la\qCopyProtect(1^\secp,\ID,\lock,\msg)$.
\end{description}

By \cref{thm:cp_to_ccobf}, $\CP$ satisfies distributional indistinguishability with respect to $D$.
From the distributional indistinguishability of $\CP$, we have $\abs{\Pr[\ttOR_3]-\Pr[\ttOR_4]}=\negl(\secp)$.

\begin{description}
\item[$\hybi{5}$:] This is the same as $\hybi{4}$ except that the re-sampling is done so that $x^*\ne \lock$.
\end{description}

Since $D$ is unpredictable, we have $\abs{\Pr[\ttOR_4]-\Pr[\ttOR_5]}=\negl(\secp)$.



$\hybi{4}$ is $\expc{\CP,\qA}{cp}{pf}{cmp}(\secp)$ where $\Dchall_{\param,\lock}$ outputs a re-sampled value $x^*\la D_\param$.
Let $\Resamp$ be the event that $\Dchall$ does re-sampling.
Also, let $\Same$ be the event that $x^*\ne\lock$ holds for re-sampled $x^*$.
Then, we have 
\ifnum\llncs=0
\begin{align}
&\advc{\CP,\qA}{cp}{pf}{cmp}(\secp)-w\\
&\le w \cdot \Pr[y_1=1\land y_2=1\mid \lnot\Resamp]+(1-w)\cdot\Pr[y_1\ne1\land y_2\ne1\mid \Resamp \land \lnot\Same]+\negl(\secp)-w\\
&\le w\cdot\Pr[y_1=1\land y_2=1\mid \lnot\Resamp]+ w\cdot(1-\Pr[y_1=1\lor y_2=1\mid \Resamp \land \lnot\Same])+\negl(\secp)-w\\
&\le w\cdot (\Pr[\ttAND_1]-\Pr[\ttOR_4])+\negl(\secp).
\end{align}
\else
\begin{align}
&\advc{\CP,\qA}{cp}{pf}{cmp}(\secp)-w\\
&\le w \cdot \Pr[y_1=1\land y_2=1\mid \lnot\Resamp]\\
&~~~~+(1-w)\cdot\Pr[y_1\ne1\land y_2\ne1\mid \Resamp \land \lnot\Same]+\negl(\secp)-w\\
&\le w\cdot\Pr[y_1=1\land y_2=1\mid \lnot\Resamp]\\
&~~~~+ w\cdot(1-\Pr[y_1=1\lor y_2=1\mid \Resamp \land \lnot\Same])+\negl(\secp)-w\\
&\le w\cdot (\Pr[\ttAND_1]-\Pr[\ttOR_4])+\negl(\secp).
\end{align}
\fi
The second inequality uses $1-w \le w$.
From the above discussions, we have $\Pr[\ttAND_1]-\Pr[\ttOR_4]\le\negl(\secp)$
Therefore, we have $\advc{\CP,\qA}{cp}{pf}{cmp}(\secp)\le w+\negl(\secp)$.
This completes the proof.
\end{proof}


\paragraph{Implication for multi-bit output point functions.}
For the case of multi-bit output point functions, we can prove that simulation-based copy-protection security implies the security definition by \cite{ARXIV:ColMajPor20} with respect to any challenge distribution considered by \cite{ARXIV:ColMajPor20}.

\begin{definition}[Copy-Protection Security for Point Functions with Unpredictable Messages]\label{def:cp_protection_point_function_umpm}
Let $D=\{D_\param\}$ be a family of distributions.
We say that a copy-protection scheme satisfies security with unpredictable messages with respect to $D$ if it satisfies copy-protection security by \cite{ARXIV:ColMajPor20} with respect to $(\delta,D,\Dmsg,\Dchall)$ for any family of unpredictable distributions $\Dmsg=\{\Dmsg_\param\}$, family of distributions $\Dchall=\{\Dchall_{\param,\lock}\}_{\param,\lock}$ such that
$$\ptrivunpm=\Pr[x_1^*\ne \lock \land x_2^*\ne \lock] + \max\{\Pr[x_1^*\ne\lock\land x_2^*=\lock],\Pr[x_2^*\ne\lock \land x_1^*=\lock]\}$$
 is fixed regardless of the value of $\params$ and $\lock$, and $\delta=\ptrivunpm$.
\end{definition}


\begin{theorem}
Let $D=\{D_\param\}$ be a family of distributions.
Assume $\CP$ satisfies simulation-based copy-protection security with respect to $D$.
Then, $\CP$ also satisfies copy-protection security for point functions with unpredictable messages with respect to $D$.
\end{theorem}
\begin{proof}
Let $\qA=(\qA_0,\qA_1,\qA_2)$ be any QPT adversary.
Also, $\Dmsg=\{\Dmsg_\param\}$ be a family of unpredictable distributions and $\Dchall=\{\Dchall_{\param,\lock}\}_{\param,\lock}$ a family of distributions such that
$$\ptrivunpm=\Pr[x_1^*\ne \lock \land x_2^*\ne \lock] + \max\{\Pr[x_1^*\ne\lock\land x_2^*=\lock],\Pr[x_2^*\ne\lock \land x_1^*=\lock]\}$$
 is fixed regardless of the value of $\params$ and $\lock$.
As shown in the proof of \cite[Theorem 1]{ARXIV:ColMajPor20}, we have
\begin{align}
\advc{\CP,\qA}{cp}{pf}{cmp}(\secp)\le\ptrivunpm+2\cdot\Pr[y_1=\msg \land y_2=\msg \mid x_1^*=\lock \land x_2^*=\lock].
\end{align}
We prove $\Pr[y_1=\msg \land y_2=\msg \mid x_1^*=\lock \land x_2^*=\lock]=\negl(\secp)$ by using the following sequence of experiments.

\begin{description}
\item[$\hybi{1}$:] This is $\expc{\CP,\qA}{cp}{pf}{cmp}(\secp)$ conditioned that $x_1^*=\lock$ and $x_2^*=\lock$.
\end{description}

We define the following two events.
\begin{description}
\item[$\ttAND_i$:]$y_1=\msg$ and $y_2=\msg$ in $\hybi{i}$.
\item[$\ttOR_i$:]$y_1=\msg$ or $y_2=\msg$ in $\hybi{i}$.
\end{description}

\begin{description}
\item[$\hybi{2}$:] This is the same as $\hybi{1}$ except that $\rho$ is generated as $\qSim(1^\secp, P.\pp,\abs{\msg})$, where $\qSim$ is the simulator that is guaranteed to exit by the simulation-based security of $\CP$.
\end{description}

We consider the following adversary $\qB=(\qB_0,\qB_1,\qB_2)$ that attacks the simulation-based security of $\CP$. $\qB_0$ behaves as follows.
\begin{enumerate}
\item $\qB_0$ obtains $\param$ from $\qA_0$, generates $\msg\la\Dmsg_\param$, and sends them to the challenger.
$\qB_0$ obtains $\rho$ from the challenger and sends it to $\qA_0$.
\item When $\qA_0$ creates a bipartite state $\qstateq$ over registers $\qreg{R}_1$ and $\qreg{R}_2$, $\qB_0$ sends $\qstateq[\qreg{R}_1]$ and $\qstateq[\qreg{R}_2]$ to $\qB_1$ and $\qB_2$, respectively.
\end{enumerate}
$\qB_\alpha$ for $\alpha\in\{1,2\}$ behaves as follows.
\begin{enumerate}
\item $\qB_\alpha$ send $\qstateq[\qreg{R}_\alpha]$ to $\qA_\alpha$.
\item When $\qB_\alpha$ obtains $\lock$ from the challenger, $\qB_\alpha$ sends it to $\qA_\alpha$.
\item When $\qA_\alpha$ output $y_\alpha$, it outputs $b_\alpha=0$ if $y_\alpha=\msg$.
\end{enumerate}

Let the challenge bit in the security game played by $\qB$ be $b$.
If $b=0$, $\qB$ perfectly simulates $\hybi{1}$ to $\qA$.
If $b=1$, $\qB$ perfectly simulates $\hybi{2}$ to $\qA$.
Also, for $\alpha\in\{1,2\}$, $\qB_\alpha$ output $0$ if and only if $y_\alpha=\msg$ holds.
Then, we have 
\begin{align}
\Pr[b_1^\prime=b_2^\prime=b]-\frac{1}{2}
&=\Pr[b_1^\prime= b_2^\prime=b=0]+\Pr[b_1^\prime= b_2^\prime=b=1]-\frac{1}{2}\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]+\Pr[b_1^\prime=1\land b_2^\prime=1\mid b=1])-\frac{1}{2}\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]-(1-\Pr[b_1^\prime=1\land b_2^\prime=1\mid b=1]))\\
&=\frac{1}{2}(\Pr[b_1^\prime=0\land b_2^\prime=0\mid b=0]-\Pr[b_1^\prime=0\lor b_2^\prime=0\mid b=1])\\
&=\frac{1}{2}(\Pr[\ttAND_1]-\Pr[\ttOR_2]).
\end{align}
Thus, from the simulation-based copy-protection security of $\CP$, we have $\Pr[\ttAND_1]-\Pr[\ttOR_2]\le\negl(\secp)$.

In $\hybi{2}$, $\qA$ is not given any information of $\msg$.
Thus, we have $\Pr[\ttOR_2]=\negl(\secp)$ since $\Dmsg$ is a family of unpredictable distributions.
From the above discussions, we obtain 
\begin{align}
\advc{\CP,\qA}{cp}{pf}{unpm}(\secp)
&\le\ptrivunpm+\Pr[\ttAND_1]\\
&\le\ptrivunpm+\Pr[\ttOR_2]+\negl(\secp)\\
&=\ptrivunpm+\negl(\secp).
\end{align}
This completes the proof.
\end{proof}







